Convergence Bounds for Sequential Monte Carlo on Multimodal Distributions using Soft Decomposition

We prove bounds on the variance of a function $f$ under the empirical measure of the samples obtained by the Sequential Monte Carlo (SMC) algorithm, with time complexity depending on local rather than global Markov chain mixing dynamics. SMC is a Markov Chain Monte Carlo (MCMC) method, which starts by drawing $N$ particles from a known distribution, and then, through a sequence of distributions, re-weights and re-samples the particles, at each instance applying a Markov chain for smoothing. In principle, SMC tries to alleviate problems from multi-modality. However, most theoretical guarantees for SMC are obtained by assuming global mixing time bounds, which are only efficient in the uni-modal setting. We show that bounds can be obtained in the truly multi-modal setting, with mixing times that depend only on local MCMC dynamics.

==> preamble.tex <==
\usepackage{parskip}
\usepackage[margin=1.0in]{geometry}

%----------------------------
% for image processing
%----------------------------

%\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{float}

%----------------------------
%  math and symbols
%----------------------------
\usepackage{physics}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amstext}
\usepackage{amssymb}
\usepackage{tabularx}

%--------------------------
% Specific Math Operators
%--------------------------
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\dx}{\mathrm{d}}
\newcommand{\e}{\mathbb{E}}
\newcommand{\rk}{\mathrm{rk}}
\newcommand{\de}{\Delta}
\newcommand{\al}{\alpha}
\newcommand{\h}{\eta}
\newcommand{\pr}{\mathbb{P}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}

%--------------------------

\usepackage[english]{babel}


% for pdf
\usepackage{pdfpages}



\usepackage{dsfont}
%\usepackage{float}
\usepackage{xcolor}
\usepackage{textcomp}
\usepackage{listings}
\usepackage{relsize}
\usepackage{multicol}
%\usepackage{subcaption}
\usepackage{hyperref}
\hypersetup{
	colorlinks=true,
	%hidelinks,
	linkcolor=black,
	filecolor=black,      
	urlcolor=black,
	citecolor=blue,
}

\usepackage{physics}
\usepackage{url}

% \usepackage{algorithm}
% \usepackage{algpseudocode}
\usepackage{pifont}

\usepackage{bbm}
\usepackage{mathtools}
\usepackage{hhline}
\usepackage{tabularx}

\theoremstyle{definition}
\newtheorem{example}{Example}[section]
\newtheorem{note}{Note}[section]
\newtheorem{question}{Question}[section]
\newtheorem{issue}{Issue}[section]


\newcommand{\tcb}[1]{\textcolor{blue}{#1}}
\newcommand{\tcr}[1]{\textcolor{red}{#1}}

\newcommand{\gak}[1]{\textcolor{red}{#1}}

\newcommand{\Ent}[2]{\operatorname{Ent}_{#2}[{#1}]}

\usepackage[ruled,vlined]{algorithm2e}

\usepackage{hyperref}
\hypersetup{
	colorlinks=true,
	%hidelinks,
	linkcolor=black,
	filecolor=black,      
	urlcolor=black,
	citecolor=blue,
}

\usepackage{tcolorbox}
\PassOptionsToPackage{svgnames}{xcolor}
\tcbuselibrary{skins,breakable}
\usetikzlibrary{shadings,shadows}
\newenvironment{myblock}[1]{%
    \tcolorbox[beamer,%
    noparskip,breakable,
    %colback=LightBlue,colframe=DarkBlue,%
    %colbacklower=DarkBlue!75!LightBlue,%
    title=#1]}%
    {\endtcolorbox}
